Hyp2Nav: Hyperbolic Planning and Curiosity for Crowd Navigation

Autonomous robots are increasingly becoming a strong fixture in social environments. Effective crowd navigation requires not only safe yet fast planning, but should also enable interpretability and computational efficiency for working in real-time on embedded devices. In this work, we advocate for hyperbolic learning to enable crowd navigation and we introduce Hyp2Nav. Different from conventional reinforcement learning-based crowd navigation methods, Hyp2Nav leverages the intrinsic properties of hyperbolic geometry to better encode the hierarchical nature of decision-making processes in navigation tasks. We propose a hyperbolic policy model and a hyperbolic curiosity module that results in effective social navigation, best success rates, and returns across multiple simulation settings, using up to 6 times fewer parameters than competitor state-of-the-art models. With our approach, it becomes even possible to obtain policies that work in 2-dimensional embedding spaces, opening up new possibilities for low-resource crowd navigation and model interpretability. Insightfully, the internal hyperbolic representation of Hyp2Nav correlates with how much attention the robot pays to the surrounding crowds, e.g. due to multiple people occluding its pathway or to a few of them showing colliding plans, rather than to its own planned route. The code is available at https://github.com/GDam90/hyp2nav.

==> Tables/comparison_stats.tex <==
\begin{table}[!b]

\centering{

\caption{
%Complex scenario (tested on 1000 random test cases)
\textbf{Comparison of the SotA methods' efficiency.} Our hyperbolic approach to crowd navigation obtains the best performance at a fraction of the required number of learnable parameters.
}
\label{tab:comparison_stats}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc} 
\toprule


 & \multicolumn{1}{c}{\scriptsize\textbf{Params.}$\downarrow$}  & \multicolumn{1}{c}{\scriptsize\textbf{Mem. Footprint (MB)} $\downarrow$}  & \multicolumn{1}{c}{\scriptsize\textbf{Runtime (msec) }$\downarrow$} & \multicolumn{1}{c}{\scriptsize\textbf{\AF{steps/second}}$\uparrow$}  \\ 
\midrule
SGD3QN-ICM \cite{martinez2023} & 361K &  1.38 & 13.4 & 74.7 \\
SGD3QN-RE3 \cite{martinez2023} & 149K &  0.57 & 12.9 &  75.9 \\
SafeCrowdNav \cite{xu2023} & 361K & 1.38 & 13.4 & 74.7 \\
\rowcolor{Gray}
\modelname-128 & 144K & 0.55 & 31.3 & 30.6 \\
\rowcolor{Gray}
\modelname & \textbf{55K} & \bf{0.21} & 30.6 & 32.0 \\

\end{tabular}
}}

\end{table}

==> Tables/comparison_with_sota_5.tex <==
\begin{table}[t]

\centering{

\caption{
Simple scenario (tested on 1000 random test cases) }
\label{tab:comparison_5h}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|ccc} 
\hline
 % &  & \multicolumn{3}{|c|}{\textbf{Simple}} \\  


 \textbf{Method} & \multicolumn{1}{|c}{\textbf{Avg. Return }$\uparrow$} & \multicolumn{1}{c}{\textbf{Nav. Time} $\downarrow$} & \multicolumn{1}{c}{\textbf{Success Rate} $\uparrow$}  \\ 
\hline\hline

ORCA\cite{van2011ORCA} & 0.323 &  13.87 & 73.6   \\
Intrinsic-SGD3QN\cite{martinez2023} & 0.696 &  \textbf{9.79} & 96.6 \\
AEMCARL\cite{wang2022adaptive} & 0.539 &  12.86 & 92.0    \\
SafeCrowdNav\cite{xu2023} & 0.707 &  9.98 & 98.6    \\
\modelname-128 & \textbf{0.747} &  10.56 & \textbf{100}  \\
\modelname-2  & 0.707 & 10.66  & 99.5   \\




\hline
\end{tabular}
}
}

\end{table}

==> Tables/comparison_with_sota_new.tex <==
\begin{table}[t]
\centering{
\caption{Complex scenario (tested on 1000 random test cases)}
\label{tab:comparison_10h}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|ccc} 
\hline
& \textbf{Method} & \multicolumn{1}{|c}{\textbf{Success Rate} $\uparrow$} & \multicolumn{1}{c}{\textbf{Nav. Time} $\downarrow$} & \multicolumn{1}{c}{\textbf{Avg. Return} $\uparrow$}  \\ 
\hline\hline

\multirow{6}{*}{Circle} & ORCA\cite{van2011ORCA} & 76.9 &  11.01 & 0.331   \\
& Intrinsic-SGD3QN-ICM\cite{martinez2023}  & 96.8 &  11.37 & 0.668  \\
& Intrinsic-SGD3QN-RE3\cite{martinez2023} & 97.1 &  11.01 & 0.682  \\
& SafeCrowdNav\cite{xu2023} & 97.7 & 11.18 & 0.673    \\
& \modelname-128 & 97.9 &  \bf{10.94} & 0.678    \\
& \modelname & \bf{99.3} &  12.04 & \textbf{0.695}   \\

\hline
\hline

\multirow{6}{*}{Square} & ORCA\cite{van2011ORCA} & 84.0 &  12.86 & 0.442 \\
& Intrinsic-SGD3QN-ICM\cite{martinez2023}  & 97.0 &  10.73 & 0.687 \\
& Intrinsic-SGD3QN-RE3\cite{martinez2023} & 95.8 &  10.22 & 0.675 \\
& SafeCrowdNav\cite{xu2023} &  97.7 &  10.54 & 0.678   \\
& \modelname-128 & 98.6  & \textbf{10.15} & 0.693     \\
& \modelname  &  \textbf{99.8} & 11.08 & \textbf{0.715}    \\

\hline
\end{tabular}
}}
\end{table}

==> Tables/main_results.tex <==
\begin{table*}[t]

\centering{

\caption{
Comparative evaluation. }
\label{tab:together}
% \resizebox{\linewidth}{
\begin{tabular}{l|c|ccc|cccc} 
\hline
 &  & \multicolumn{3}{|c|}{\textbf{Circle}}  & \multicolumn{3}{c}{\textbf{Square}} \\ 


 & \textbf{Dimension} & \multicolumn{1}{|c}{\textbf{Avg. Return}} & \multicolumn{1}{c}{\textbf{Nav. Time}} & \multicolumn{1}{c|}{\textbf{Success Rate}}  & \textbf{Avg. Return} & \multicolumn{1}{c}{\textbf{Nav. Time}} & \multicolumn{1}{c}{\textbf{Success Rate}} \\ 
\hline\hline

\multirow{1}{*}{Paper Results} & 128 & 0.668 & 11.37 & 96.8 & 0.687 & 10.73 & 97.0\\


\multirow{1}{*}{Euclidean} & 2 & 0.721 & 11.14 & 99.7 & 0.697 & 10.51 & 97.4 \\

% \multirow{1}{*}{Euclidean}  & 16 & 0.702 & 12.0 & 98.4 &  &  & \\

\multirow{1}{*}{Euclidean}  & 32 & 0.713 & 10.13 & 98.8 & 0.701 & 9.47  & 97.2 \\

\multirow{1}{*}{Euclidean} & 64 & 0.729 & 10.33 & 99.3 & 0.702 & 10.18 & 98.1 \\

\multirow{1}{*}{Euclidean - replicated res.} & 128 & 0.718 & 10.50 & 98.0 &  &  & \\

\hline

\multirow{1}{*}{HICM} & 2 & 0.737 & \textbf{9.76} & 99.4 & 0.747 & 9.14 & 99.0 \\

\multirow{1}{*}{HICM} & 32 & 0.728 & 9.91 & 99.4 & 0.746 & 9.23 & 99.3 \\

\multirow{1}{*}{HICM} & 64 & 0.734 & 9.83 & 99.4 & 0.740 & \textbf{9.07} & 98.6 \\

\multirow{1}{*}{HICM} & 128 & 0.745 & 10.02 & 99.5 & \textbf{0.755} & 9.28 & \textbf{99.6} \\
    

\hline

\multirow{1}{*}{HHICM} & 2 & 0.707 & 10.66 & 99.5 & 0.739 & 9.33 & 99.1 \\

\multirow{1}{*}{HHICM} & 32 & 0.728 & 10.46 & 99.4 &  &  &\\

\multirow{1}{*}{HHICM} & 64 & 0.675 & 11.32 & 99.1 & 0.721 & 9.87 & 99.8 \\

\multirow{1}{*}{HHICM} & 128 & \textbf{0.747} & 10.56 & \textbf{100} & 0.754 & 9.42 & \textbf{99.6} \\


   
\hline
\end{tabular}
}
% }

\end{table*}

==> Tables/main_results_10H.tex <==
% \begin{table}[t]

% \centering{

% \caption{
% Ablation, CIRCLE, Trained on 10 humans, }
% \label{tab:together_10H}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|ccc} 
% \hline
%  % &  & \multicolumn{3}{|c|}{\textbf{Circle}}  & \multicolumn{3}{c}{\textbf{Square}} \\ 


%  \textbf{Emb. Dim.} & \textbf{Method} & \multicolumn{1}{|c}{\textbf{Avg. Return} $\uparrow$} & \multicolumn{1}{c}{\textbf{Nav. Time} $\downarrow$} & \multicolumn{1}{c}{\textbf{Success Rate} $\uparrow$}   \\ 
% \hline\hline


%  \multirow{3}{*}{2 } & \multirow{1}{*}{Intrinsic-SGD3QN~\cite{martinez2023}  }  & -0.03 &  14.81 & 63.3   \\
% &\multirow{1}{*}{\modelname w/o \HICM}  & \textcolor{black}{\textbf{0.698}} & \textcolor{black}{\textbf{11.58}}  & 98.9   \\
% &\multirow{1}{*}{\modelname}  & 0.695 &  12.04 & \textcolor{ForestGreen}{\bf{99.3}}   \\

% \hline

% \multirow{3}{*}{32 }  & \multirow{1}{*}{Intrinsic-SGD3QN~\cite{martinez2023}  }  &  0.693 & 11.29  & 98.9  \\
% &\multirow{1}{*}{\modelname w/o \HICM}  & 0.609 &  14.35 &  96.5 \\
% &\multirow{1}{*}{\modelname}  & \textcolor{ForestGreen}{\bf{0.714}} &  \textcolor{black}{\textbf{11.14}} &  \textcolor{black}{\bf{99.0}} \\

% \hline

%  \multirow{3}{*}{64 }  & \multirow{1}{*}{Intrinsic-SGD3QN~\cite{martinez2023} } & 0.669 & 11.57  & 98.3   \\
% &\multirow{1}{*}{\modelname w/o \HICM}  & 0.686 & 11.24  & 98.3    \\
% &\multirow{1}{*}{\modelname}  & \textcolor{black}{\bf{0.699}} & \textcolor{black}{\textbf{11.16}}  & \textcolor{black}{\textbf{98.8}}  \\

% % \multirow{1}{*}{Intrinsic-SGD3QN} & 128 & 0.673 &  10.85 &  96.9 \\
% \hline

% \multirow{3}{*}{128 } & \multirow{1}{*}{Intrinsic-SGD3QN~\cite{martinez2023}}  & 0.668 & 11.37 & 96.8 \\
% &\multirow{1}{*}{\modelname w/o \HICM} &   \textcolor{black}{\textbf{0.685}} &  \textcolor{ForestGreen}{\bf{10.76}} & \textcolor{black}{\textbf{98.0}}   \\
% &\multirow{1}{*}{\modelname} &   0.678 &  10.94 & 97.9   \\

% % \hline

% % \multirow{1}{*}{HICM} & 2 & \textbf{0.717} & 11.59  &  \textbf{99.7}   \\

% % \multirow{1}{*}{HICM} & 32 & 0.684 & 11.07  & 98.7  \\

% % \multirow{1}{*}{HICM} & 64 & 0.695 &  11.17 &  98.8    \\

% % \multirow{1}{*}{HICM} & 128 & 0.693 & \textbf{10.76}  & 98.5 \\
% \hline
% \hline
% \end{tabular}
% }}
% % }

% \end{table}




\begin{table}[t]

\centering{

\caption{
Ablation, CIRCLE, Trained on 10 humans, \PM{Better as a bar plot with only 128 and 2? And optionally 4 and 8.} }
\label{tab:together_10H}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|ccc} 
\toprule
 % &  & \multicolumn{3}{|c|}{\textbf{Circle}}  & \multicolumn{3}{c}{\textbf{Square}} \\ 


 \textbf{Dim.} & \textbf{Method} & \multicolumn{1}{c}{\textbf{Nav. Time} $\downarrow$}  & \multicolumn{1}{c}{\textbf{Avg. Return} $\uparrow$}& \multicolumn{1}{c}{\textbf{Success Rate} $\uparrow$}   \\ 

\hline

\multirow{3}{*}{128 } & \multirow{1}{*}{SGD3QN~\cite{martinez2023}}  & 11.37 & 0.668 & 96.8 \\
&\multirow{1}{*}{\modelname w/o \HICM} &  \textcolor{ForestGreen}{\bf{10.76}} &   \textcolor{black}{\textbf{0.685}}  & \textcolor{black}{\textbf{98.0}}   \\
&\multirow{1}{*}{\modelname} &  10.94 &   0.678  & 97.9   \\

\hline

\multirow{3}{*}{64 }  & \multirow{1}{*}{SGD3QN~\cite{martinez2023} } & 11.57 & 0.669  & 98.3   \\
&\multirow{1}{*}{
\modelname w/o \HICM
} & 11.24 & 0.686   & 98.3    \\
&\multirow{1}{*}{\modelname} & \textcolor{black}{\textbf{11.16}}  & \textcolor{black}{\bf{0.699}}  & \textcolor{black}{\textbf{98.8}}  \\

\hline

\multirow{3}{*}{32 }  & \multirow{1}{*}{SGD3QN~\cite{martinez2023}  } & 11.29 &  0.693   & 98.9  \\
&\multirow{1}{*}{\modelname w/o \HICM}  &  14.35 & 0.609 &  96.5 \\
&\multirow{1}{*}{\modelname} &  \textcolor{black}{\textbf{11.14}} & \textcolor{ForestGreen}{\bf{0.714}}  &  \textcolor{black}{\bf{99.0}} \\

% \multirow{1}{*}{Intrinsic-SGD3QN} & 128 & 0.673 &  10.85 &  96.9 \\
% \hline

% \multirow{3}{*}{8 } & \multirow{1}{*}{Intrinsic-SGD3QN~\cite{martinez2023}  }  &  10.94  & 0.717  & 98.9   \\
% &\multirow{1}{*}{\modelname w/o \HICM} & 11.04   & 0.667 & 97.0   \\
% &\multirow{1}{*}{\modelname}  &  11.03 & 0.679 & 98.8   \\


% \hline

% \multirow{3}{*}{4 } & \multirow{1}{*}{Intrinsic-SGD3QN~\cite{martinez2023}  }  &  11.46  & 0.706  & 99.0   \\
% &\multirow{1}{*}{\modelname w/o \HICM} &    &  &    \\
% &\multirow{1}{*}{\modelname}  &   &  &    \\


\hline

\multirow{3}{*}{2 } & \multirow{1}{*}{SGD3QN~\cite{martinez2023}  }  &  14.81  & -0.03& 63.3   \\
&\multirow{1}{*}{\modelname w/o \HICM} & \textcolor{black}{\textbf{11.58}}   & {0.695} & 98.9   \\
&\multirow{1}{*}{\modelname}  &  12.04  &\textcolor{black}{ \textbf{0.698}} & \textcolor{ForestGreen}{\bf{99.3}}   \\


% \hline

% \multirow{1}{*}{HICM} & 2 & \textbf{0.717} & 11.59  &  \textbf{99.7}   \\

% \multirow{1}{*}{HICM} & 32 & 0.684 & 11.07  & 98.7  \\

% \multirow{1}{*}{HICM} & 64 & 0.695 &  11.17 &  98.8    \\

% \multirow{1}{*}{HICM} & 128 & 0.693 & \textbf{10.76}  & 98.5 \\
\bottomrule
\end{tabular}
}}
% }

\end{table}

==> Tables/main_results_10H_new.tex <==
\begin{table}[t]
\centering{
\caption{Ablation, CIRCLE, Trained on 10 humans}
\label{tab:together_10H}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|ccc} 
\hline

\textbf{Emb. Dim.} & \textbf{Method} & \multicolumn{1}{|c}{\textbf{Success Rate} $\uparrow$} & \multicolumn{1}{c}{\textbf{Nav. Time} $\downarrow$} & \multicolumn{1}{c}{\textbf{Avg. Return} $\uparrow$}   \\ 
\hline\hline

\multirow{3}{*}{128 } & Intrinsic-SGD3QN~\cite{martinez2023}  & 96.8 & 11.37 & 0.668 \\
& \modelname w/o \HICM &  \textbf{98.0} &  \textcolor{ForestGreen}{\bf{10.76}} & \textbf{0.685}   \\
& \modelname &  97.9 &  10.94 & 0.678   \\

\hline

\multirow{3}{*}{64 } & Intrinsic-SGD3QN~\cite{martinez2023}  & 98.3 & 11.57  & 0.669   \\
& \modelname w/o \HICM  & 98.3 & 11.24  & 0.686    \\
& \modelname  & \textbf{98.8} & \textbf{11.16}  & \textbf{0.699}  \\

\hline

\multirow{3}{*}{32 } & Intrinsic-SGD3QN~\cite{martinez2023}   & 98.9 & 11.29  & 0.693  \\
& \modelname w/o \HICM  & 96.5 &  14.35 & 0.609 \\
& \modelname  & \bf{99.0} &  \textbf{11.14} & \textcolor{ForestGreen}{\bf{0.714}} \\

\hline

\multirow{3}{*}{2 } & Intrinsic-SGD3QN~\cite{martinez2023}   & 63.3 &  14.81 & -0.03   \\
& \modelname w/o \HICM  & 98.9 & \textbf{11.58}  & \textbf{0.698}   \\
& \modelname  & \textcolor{ForestGreen}{\bf{99.3}} &  12.04 & 0.695   \\

\hline
\hline
\end{tabular}
}}
\end{table}

==> Tables/main_results_10H_temp.tex <==
\begin{table*}[t]

\centering{

\caption{
Trained on 10, tested on 10 }
\label{tab:together_10H}
% \resizebox{\linewidth}{
\begin{tabular}{l|c|ccc|cccc} 
\hline
 &  & \multicolumn{3}{|c|}{\textbf{Circle}}  & \multicolumn{3}{c}{\textbf{Square}} \\ 


 & \textbf{Dimension} & \multicolumn{1}{|c}{\textbf{Avg. Return}} & \multicolumn{1}{c}{\textbf{Nav. Time}} & \multicolumn{1}{c|}{\textbf{Success Rate}}  & \textbf{Avg. Return} & \multicolumn{1}{c}{\textbf{Nav. Time}} & \multicolumn{1}{c}{\textbf{Success Rate}} \\ 
\hline\hline

% \multirow{1}{*}{Euclidean 60} & 2 & -0.372 &  15.08 & 13.6  &   &  &  \\

% \multirow{1}{*}{Euclidean 60} & 32 & 0.607 & 12.55  & 95.7  &   &  &  \\

% \multirow{1}{*}{Euclidean 60} & 64 & 0.630 & 10.94  & 95.7  &   &  &  \\

% \multirow{1}{*}{Euclidean 60} & 128 & 0.571 & 11.65  & 91.6   &   &  &  \\
    

% \hline



\multirow{1}{*}{Euclidean  } & 2 & -0.03 &  14.81 & 63.3   &  0.207 & 14.13 & 80.3 \\

\multirow{1}{*}{Euclidean  }  & 32 & 0.693 & 11.29  & 98.9  &  0.724 & 10.25 & 99.4 \\

\multirow{1}{*}{Euclidean  } & 64 & 0.669 & 11.57  & 98.3  & 0.707  & 10.53 & 99.2 \\

\multirow{1}{*}{Euclidean  - replicated res.} & 128 & 0.673 &  10.85 &  96.9 &  0.718 & \textbf{9.95} & 98.9 \\

\multirow{1}{*}{Paper Results} & 128 & 0.668 & 11.37 & 96.8 & 0.687 & 10.73 & 97.0\\

\hline

\multirow{1}{*}{HICM} & 2 & \textbf{0.717} & 11.59  &  \textbf{99.7} &  \ul{0.726} & 10.74 & \ul{99.7} \\

\multirow{1}{*}{HICM} & 32 & 0.684 & 11.07  & 98.7  &  0.720 & 10.15 & 99.4 \\

\multirow{1}{*}{HICM} & 64 & 0.695 &  11.17 &  98.8  &  \ul{0.726} & 10.15 & 99.5  \\

\multirow{1}{*}{HICM} & 128 & 0.693 & \textbf{10.76}  & 98.5 & 0.717  & \textbf{9.95} & 99.1   \\
    
\hline

\multirow{1}{*}{HyperVnet  } & 2 & 0.698 & 11.58  & 98.9  &  0.715 & 10.65 & 99.3 \\

\multirow{1}{*}{HyperVnet  } & 32 &  &   &   &   &  &  \\

\multirow{1}{*}{HyperVnet  } & 64 &  &   &   &   &  &  \\

\multirow{1}{*}{HyperVnet  } & 128 & 0.685 &  10.76 & 98.0  &   &  &  \\

\hline

\multirow{1}{*}{HyperVnet  + HICM} & 2 & 0.695 &  12.04 & \ul{99.3}  &  0.715 & 11.08 & \textbf{99.8} \\

\multirow{1}{*}{HyperVnet  + HICM} & 32 & \ul{0.714} &  11.14 &  99.0 &  \textbf{0.735} & \ul{10.05} & 99.2 \\

\multirow{1}{*}{HyperVnet  + HICM} & 64 & 0.699 & 11.16  &  98.8 & 0.717 & 10.37  & \ul{99.7} \\

\multirow{1}{*}{HyperVnet  + HICM} & 128 & 0.678 &  \ul{10.94} & 97.9  & -0.15  & 18.2 & 36.7 \\


\hline
\end{tabular}
}
% }

\end{table*}

==> Tables/main_results_20H_new.tex <==
\begin{table}[t]
\centering{
\caption{Trained on 10 H, tested on 20 H, CIRCLE, 2-dim embeddings}
\label{tab:together_20H}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc} 
\hline
& \multicolumn{1}{|c}{\textbf{Success Rate} $\uparrow$} & \multicolumn{1}{c}{\textbf{Nav. Time} $\downarrow$} & \multicolumn{1}{c}{\textbf{Avg. Return} $\uparrow$}   \\ 
\hline\hline

\multirow{1}{*}{Intrinsic-SGD3QN~\cite{martinez2023}}  & 93.2 & \textbf{13.81} & 0.559  \\
SafeCrowdNav\cite{xu2023} & 90.6 & 13.86 & 0.478  \\
\multirow{1}{*}{\modelname w/o \HICM}  & \textbf{94.6} & 14.78 & 0.560      \\
\multirow{1}{*}{\modelname} & \textbf{94.6} & 14.55 & \textbf{0.571}   \\

\hline
\end{tabular}
}}
\end{table}

==> Tables/main_results_20H_temp.tex <==
\begin{table*}[t]

\centering{

\caption{
Trained on 10, tested on 20 }
\label{tab:together_20H}
% \resizebox{\linewidth}{
\begin{tabular}{l|ccc|cccc} 
\hline
 &   \multicolumn{3}{|c|}{\textbf{Circle}}  & \multicolumn{3}{c}{\textbf{Square}} \\ 


  & \multicolumn{1}{|c}{\textbf{Avg. Return}} & \multicolumn{1}{c}{\textbf{Nav. Time}} & \multicolumn{1}{c|}{\textbf{Success Rate}}  & \textbf{Avg. Return} & \multicolumn{1}{c}{\textbf{Nav. Time}} & \multicolumn{1}{c}{\textbf{Success Rate}} \\ 
\hline\hline


% \multirow{1}{*}{Euclidean 360} & 2 &  &   &    &    &   &   \\

% \multirow{1}{*}{Euclidean 360}  & 32 &  &   &    &    &   &   \\

% \multirow{1}{*}{Euclidean 360} & 64 &  &   &    &    &   &   \\

\multirow{1}{*}{Euclidean }  & 0.559 &  13.81 &  93.2  &  0.570  & \textbf{13.22}  &  93.5 \\

% \hline

\multirow{1}{*}{HICM}  & 0.626 &  14.37 & 96.4   & \textbf{0.625}  & 14.06  & \textbf{97.1}   \\

% \multirow{1}{*}{HICM} & 32 &  &   &    &    &   &   \\

% \multirow{1}{*}{HICM} & 64 &  &   &    &    &   &   \\

% \multirow{1}{*}{HICM} & 128 &  &   &    &    &   &   \\
    

% \hline

\multirow{1}{*}{HyperVnet  + HICM} &  &   &    &  0.591  & 14.22  & 96.1  \\

% \multirow{1}{*}{HHICM} & 32 &  &   &    &    &   &   \\

% \multirow{1}{*}{HHICM} & 64 &  &   &    &    &   &   \\

% \multirow{1}{*}{HHICM} & 128 &  &   &    &    &   &   \\


\hline
\end{tabular}
}
% }

\end{table*}
